From JPEG to CUDA Batch: Measuring RGB Input Pipeline Throughput

We measure how many ready batches per second eight image input pipelines deliver to an NVIDIA L4. Each pipeline starts with RGB JPEG files and delivers synchronized CUDA float16 batches of 256 images. The benchmark contains 1314 measurements across 73 recipes. On the 34 recipes shared by all eight paths, DALI delivered a median of 19.7 batches/s and AlbumentationsX (AX) delivered 17.1. DALI was fastest on 34 of those recipes. Median peak process GPU memory was 1,872 MiB for DALI and 404 MiB for AX.

==> generated/coverage-mapping.tex <==
% Generated by paper/generate_results.py. Do not edit by hand.
Additive\allowbreak{}Noise & --- & --- & --- \\
Advanced\allowbreak{}Blur & --- & --- & --- \\
Affine & Random\allowbreak{}Affine /\allowbreak{} Random\allowbreak{}Shear & Random\allowbreak{}Affine & Image.\allowbreak{}transform(\allowbreak{}AFFINE)\allowbreak{} \\
At\allowbreak{}Least\allowbreak{}One\allowbreak{}BBox\allowbreak{}Random\allowbreak{}Crop & --- & Random\allowbreak{}Io\allowbreak{}UCrop & --- \\
Atmospheric\allowbreak{}Fog & --- & --- & --- \\
Auto\allowbreak{}Contrast & Random\allowbreak{}Auto\allowbreak{}Contrast & Random\allowbreak{}Autocontrast & Image\allowbreak{}Ops.\allowbreak{}autocontrast \\
BBox\allowbreak{}Safe\allowbreak{}Random\allowbreak{}Crop & --- & --- & --- \\
BBox\allowbreak{}Subset\allowbreak{}Safe\allowbreak{}Random\allowbreak{}Crop & --- & --- & --- \\
Bias\allowbreak{}Field & --- & --- & --- \\
Blur & Random\allowbreak{}Box\allowbreak{}Blur & --- & Image\allowbreak{}Filter.\allowbreak{}Box\allowbreak{}Blur \\
CLAHE & Random\allowbreak{}Clahe & --- & --- \\
Center\allowbreak{}Crop & Center\allowbreak{}Crop & Center\allowbreak{}Crop & Image.\allowbreak{}crop \\
Channel\allowbreak{}Dropout & Random\allowbreak{}Channel\allowbreak{}Dropout & --- & Image.\allowbreak{}split + Image.\allowbreak{}new + Image.\allowbreak{}merge \\
Channel\allowbreak{}Shuffle & Random\allowbreak{}Channel\allowbreak{}Shuffle & Random\allowbreak{}Channel\allowbreak{}Permutation & Image.\allowbreak{}split + Image.\allowbreak{}merge \\
Channel\allowbreak{}Swap & color.\allowbreak{}rgb\_\allowbreak{}to\_\allowbreak{}bgr & functional.\allowbreak{}permute\_\allowbreak{}channels & Image.\allowbreak{}split + Image.\allowbreak{}merge \\
Chromatic\allowbreak{}Aberration & --- & --- & --- \\
Coarse\allowbreak{}Dropout & Random\allowbreak{}Erasing & Random\allowbreak{}Erasing & Image.\allowbreak{}paste \\
Color\allowbreak{}Jitter & Color\allowbreak{}Jitter /\allowbreak{} Color\allowbreak{}Jiggle & Color\allowbreak{}Jitter & --- \\
Colorize & color.\allowbreak{}Apply\allowbreak{}Color\allowbreak{}Map & --- & Image\allowbreak{}Ops.\allowbreak{}colorize \\
Constrained\allowbreak{}Coarse\allowbreak{}Dropout & --- & --- & --- \\
Copy\allowbreak{}And\allowbreak{}Paste & --- & --- & --- \\
Crop & geometry.\allowbreak{}transform.\allowbreak{}crop\_\allowbreak{}by\_\allowbreak{}indices & functional.\allowbreak{}crop & Image.\allowbreak{}crop \\
Crop\allowbreak{}And\allowbreak{}Pad & --- & functional.\allowbreak{}crop + Pad & Image.\allowbreak{}crop + Image\allowbreak{}Ops.\allowbreak{}expand \\
Crop\allowbreak{}Non\allowbreak{}Empty\allowbreak{}Mask\allowbreak{}If\allowbreak{}Exists & --- & --- & --- \\
D4 & --- & --- & --- \\
Defocus & --- & --- & --- \\
Dithering & --- & --- & Image.\allowbreak{}convert(\allowbreak{}"L")\allowbreak{}.\allowbreak{}convert(\allowbreak{}"1",\allowbreak{} dither=\allowbreak{}FLOYDSTEINBERG)\allowbreak{}.\allowbreak{}convert(\allowbreak{}"RGB")\allowbreak{} \\
Downscale & --- & --- & --- \\
Elastic\allowbreak{}Transform & Random\allowbreak{}Elastic\allowbreak{}Transform & Elastic\allowbreak{}Transform & --- \\
Emboss & filters.\allowbreak{}filter2d & --- & Image\allowbreak{}Filter.\allowbreak{}Kernel \\
Enhance & --- & --- & Image\allowbreak{}Filter.\allowbreak{}EDGE\_\allowbreak{}ENHANCE\_\allowbreak{}MORE /\allowbreak{} Image\allowbreak{}Filter.\allowbreak{}DETAIL \\
Equalize & Random\allowbreak{}Equalize & Random\allowbreak{}Equalize & Image\allowbreak{}Ops.\allowbreak{}equalize \\
Erasing & Random\allowbreak{}Erasing & Random\allowbreak{}Erasing & --- \\
Exposure\allowbreak{}Matching & --- & --- & --- \\
FDA & --- & --- & --- \\
Fancy\allowbreak{}PCA & --- & --- & --- \\
Film\allowbreak{}Grain & --- & --- & --- \\
Gauss\allowbreak{}Noise & Random\allowbreak{}Gaussian\allowbreak{}Noise & Gaussian\allowbreak{}Noise & --- \\
Gaussian\allowbreak{}Blur & Random\allowbreak{}Gaussian\allowbreak{}Blur & Gaussian\allowbreak{}Blur & Image\allowbreak{}Filter.\allowbreak{}Gaussian\allowbreak{}Blur \\
Gibbs\allowbreak{}Ringing & --- & --- & --- \\
Glass\allowbreak{}Blur & --- & --- & --- \\
Grid\allowbreak{}Distortion & --- & --- & --- \\
Grid\allowbreak{}Dropout & --- & --- & --- \\
Grid\allowbreak{}Elastic\allowbreak{}Deform & --- & --- & --- \\
Grid\allowbreak{}Mask & --- & --- & --- \\
Guided\allowbreak{}Coarse\allowbreak{}Dropout & --- & --- & --- \\
HEStain & --- & --- & --- \\
Halftone & --- & --- & --- \\
Histogram\allowbreak{}Matching & contrib.\allowbreak{}histogram\_\allowbreak{}matching & --- & --- \\
Horizontal\allowbreak{}Flip & Random\allowbreak{}Horizontal\allowbreak{}Flip & Random\allowbreak{}Horizontal\allowbreak{}Flip & Image.\allowbreak{}transpose(\allowbreak{}FLIP\_\allowbreak{}LEFT\_\allowbreak{}RIGHT)\allowbreak{} \\
Hue\allowbreak{}Saturation\allowbreak{}Value & --- & Color\allowbreak{}Jitter & --- \\
ISONoise & --- & --- & --- \\
Illumination & Random\allowbreak{}Linear\allowbreak{}Illumination /\allowbreak{} Random\allowbreak{}Linear\allowbreak{}Corner\allowbreak{}Illumination /\allowbreak{} Random\allowbreak{}Gaussian\allowbreak{}Illumination & --- & --- \\
Image\allowbreak{}Compression & Random\allowbreak{}JPEG & JPEG & JPEG save/\allowbreak{}load roundtrip \\
Invert\allowbreak{}Img & Random\allowbreak{}Invert & Random\allowbreak{}Invert & Image\allowbreak{}Ops.\allowbreak{}invert \\
KSpace\allowbreak{}Spike\allowbreak{}Noise & --- & --- & --- \\
Lens\allowbreak{}Flare & --- & --- & --- \\
Letter\allowbreak{}Box & --- & --- & Image\allowbreak{}Ops.\allowbreak{}pad \\
Longest\allowbreak{}Max\allowbreak{}Size & Longest\allowbreak{}Max\allowbreak{}Size & Resize(\allowbreak{}size=\allowbreak{}None,\allowbreak{} max\_\allowbreak{}size=\allowbreak{}.\allowbreak{}.\allowbreak{}.\allowbreak{})\allowbreak{} & Image\allowbreak{}Ops.\allowbreak{}contain \\
Mask\allowbreak{}Dropout & --- & --- & --- \\
Median\allowbreak{}Blur & Random\allowbreak{}Median\allowbreak{}Blur & --- & Image\allowbreak{}Filter.\allowbreak{}Median\allowbreak{}Filter \\
Mode\allowbreak{}Filter & --- & --- & Image\allowbreak{}Filter.\allowbreak{}Mode\allowbreak{}Filter \\
Morphological & morphology.\allowbreak{}dilation /\allowbreak{} morphology.\allowbreak{}erosion & --- & Image\allowbreak{}Filter.\allowbreak{}Max\allowbreak{}Filter /\allowbreak{} Image\allowbreak{}Filter.\allowbreak{}Min\allowbreak{}Filter \\
Mosaic & Random\allowbreak{}Mosaic & --- & --- \\
Motion\allowbreak{}Blur & Random\allowbreak{}Motion\allowbreak{}Blur & --- & --- \\
Multiplicative\allowbreak{}Noise & --- & --- & --- \\
Normalize & Normalize & Normalize & --- \\
Optical\allowbreak{}Distortion & Random\allowbreak{}Fisheye & --- & --- \\
Overlay\allowbreak{}Elements & --- & --- & --- \\
Pad & --- & Pad & Image\allowbreak{}Ops.\allowbreak{}expand \\
Pad\allowbreak{}If\allowbreak{}Needed & Pad\allowbreak{}To & Pad & Image\allowbreak{}Ops.\allowbreak{}expand \\
Perspective & Random\allowbreak{}Perspective & Random\allowbreak{}Perspective & --- \\
Photo\allowbreak{}Metric\allowbreak{}Distort & --- & Random\allowbreak{}Photometric\allowbreak{}Distort & --- \\
Piecewise\allowbreak{}Affine & --- & --- & --- \\
Pixel\allowbreak{}Distribution\allowbreak{}Adaptation & --- & --- & --- \\
Pixel\allowbreak{}Dropout & --- & --- & --- \\
Pixel\allowbreak{}Spread & --- & --- & Image.\allowbreak{}effect\_\allowbreak{}spread \\
Planckian\allowbreak{}Jitter & Random\allowbreak{}Planckian\allowbreak{}Jitter & --- & --- \\
Plasma\allowbreak{}Brightness\allowbreak{}Contrast & Random\allowbreak{}Plasma\allowbreak{}Brightness /\allowbreak{} Random\allowbreak{}Plasma\allowbreak{}Contrast & --- & --- \\
Plasma\allowbreak{}Shadow & Random\allowbreak{}Plasma\allowbreak{}Shadow & --- & --- \\
Posterize & Random\allowbreak{}Posterize & Random\allowbreak{}Posterize & Image\allowbreak{}Ops.\allowbreak{}posterize \\
RGBShift & Random\allowbreak{}RGBShift & --- & Image.\allowbreak{}point \\
Random\allowbreak{}Brightness\allowbreak{}Contrast & Random\allowbreak{}Brightness /\allowbreak{} Random\allowbreak{}Contrast & Color\allowbreak{}Jitter & Image\allowbreak{}Enhance.\allowbreak{}Brightness /\allowbreak{} Image\allowbreak{}Enhance.\allowbreak{}Contrast \\
Random\allowbreak{}Crop & Random\allowbreak{}Crop & Random\allowbreak{}Crop & Image.\allowbreak{}crop + Image\allowbreak{}Ops.\allowbreak{}expand \\
Random\allowbreak{}Crop\allowbreak{}From\allowbreak{}Borders & --- & --- & --- \\
Random\allowbreak{}Crop\allowbreak{}Near\allowbreak{}BBox & --- & --- & --- \\
Random\allowbreak{}Fog & --- & --- & --- \\
Random\allowbreak{}Gamma & Random\allowbreak{}Gamma & functional.\allowbreak{}adjust\_\allowbreak{}gamma & Image.\allowbreak{}point \\
Random\allowbreak{}Gravel & --- & --- & --- \\
Random\allowbreak{}Grid\allowbreak{}Shuffle & Random\allowbreak{}Jigsaw & --- & --- \\
Random\allowbreak{}Rain & Random\allowbreak{}Rain & --- & --- \\
Random\allowbreak{}Resized\allowbreak{}Crop & Random\allowbreak{}Resized\allowbreak{}Crop & Random\allowbreak{}Resized\allowbreak{}Crop & Image.\allowbreak{}crop + Image.\allowbreak{}transform(\allowbreak{}AFFINE)\allowbreak{} \\
Random\allowbreak{}Rotate90 & Random\allowbreak{}Rotation90 & --- & Image.\allowbreak{}transpose(\allowbreak{}ROTATE\_\allowbreak{}90)\allowbreak{} \\
Random\allowbreak{}Scale & geometry.\allowbreak{}transform.\allowbreak{}resize & Scale\allowbreak{}Jitter /\allowbreak{} Random\allowbreak{}Resize & Image.\allowbreak{}transform(\allowbreak{}AFFINE)\allowbreak{} \\
Random\allowbreak{}Shadow & --- & --- & --- \\
Random\allowbreak{}Sized\allowbreak{}BBox\allowbreak{}Safe\allowbreak{}Crop & --- & --- & --- \\
Random\allowbreak{}Sized\allowbreak{}Crop & Random\allowbreak{}Resized\allowbreak{}Crop & Random\allowbreak{}Resized\allowbreak{}Crop & Image.\allowbreak{}crop + Image.\allowbreak{}transform(\allowbreak{}AFFINE)\allowbreak{} \\
Random\allowbreak{}Snow & Random\allowbreak{}Snow & --- & --- \\
Random\allowbreak{}Sun\allowbreak{}Flare & --- & --- & --- \\
Random\allowbreak{}Tone\allowbreak{}Curve & --- & --- & --- \\
Resize & Resize & Resize & Image.\allowbreak{}resize \\
Rician\allowbreak{}Noise & --- & --- & --- \\
Ringing\allowbreak{}Overshoot & --- & --- & --- \\
Rotate & Random\allowbreak{}Rotation & Random\allowbreak{}Rotation & Image.\allowbreak{}rotate \\
Safe\allowbreak{}Rotate & --- & --- & --- \\
Salt\allowbreak{}And\allowbreak{}Pepper & Random\allowbreak{}Salt\allowbreak{}And\allowbreak{}Pepper\allowbreak{}Noise & --- & --- \\
Sharpen & Random\allowbreak{}Sharpness & Random\allowbreak{}Adjust\allowbreak{}Sharpness & Image\allowbreak{}Enhance.\allowbreak{}Sharpness \\
Shift\allowbreak{}Scale\allowbreak{}Rotate & Random\allowbreak{}Affine & Random\allowbreak{}Affine & Image.\allowbreak{}transform(\allowbreak{}AFFINE)\allowbreak{} \\
Shot\allowbreak{}Noise & --- & --- & --- \\
Smallest\allowbreak{}Max\allowbreak{}Size & Smallest\allowbreak{}Max\allowbreak{}Size & Resize(\allowbreak{}size=\allowbreak{}.\allowbreak{}.\allowbreak{}.\allowbreak{})\allowbreak{} /\allowbreak{} Random\allowbreak{}Shortest\allowbreak{}Size & Image\allowbreak{}Ops.\allowbreak{}cover \\
Solarize & Random\allowbreak{}Solarize & Random\allowbreak{}Solarize & Image\allowbreak{}Ops.\allowbreak{}solarize \\
Spatter & --- & --- & --- \\
Square\allowbreak{}Symmetry & --- & --- & --- \\
Stochastic\allowbreak{}Convolution & --- & --- & --- \\
Superpixels & --- & --- & --- \\
Thin\allowbreak{}Plate\allowbreak{}Spline & Random\allowbreak{}Thin\allowbreak{}Plate\allowbreak{}Spline & --- & --- \\
To\allowbreak{}Gray & Random\allowbreak{}Grayscale & Grayscale & Image\allowbreak{}Ops.\allowbreak{}grayscale(\allowbreak{}.\allowbreak{}.\allowbreak{}.\allowbreak{})\allowbreak{}.\allowbreak{}convert(\allowbreak{}"RGB")\allowbreak{} \\
To\allowbreak{}Sepia & --- & --- & --- \\
Transpose & --- & --- & Image.\allowbreak{}transpose(\allowbreak{}TRANSPOSE)\allowbreak{} \\
Unsharp\allowbreak{}Mask & --- & --- & Image\allowbreak{}Filter.\allowbreak{}Unsharp\allowbreak{}Mask \\
Vertical\allowbreak{}Flip & Random\allowbreak{}Vertical\allowbreak{}Flip & Random\allowbreak{}Vertical\allowbreak{}Flip & Image.\allowbreak{}transpose(\allowbreak{}FLIP\_\allowbreak{}TOP\_\allowbreak{}BOTTOM)\allowbreak{} \\
Vignetting & --- & --- & --- \\
Water\allowbreak{}Refraction & --- & --- & --- \\
XYMasking & --- & --- & --- \\
Zoom\allowbreak{}Blur & --- & --- & --- \\


==> generated/coverage.tex <==
% Generated by paper/generate_results.py. Do not edit by hand.
AlbumentationsX & 125 & 2.6.2 \\
Kornia & 57 & 0.9.0 \\
TorchVision & 40 & 0.29.2 \\
Pillow & 46 & 13.0.0 \\


==> generated/delivery-rows.tex <==
% Generated by paper/generate_results.py. Do not edit by hand.
\def\DeliveryTopRow{7}
\def\DeliveryAXRate{17.12548000}
\def\DeliveryRows{%
\DeliveryRow{0}{Kornia CPU}{7.89020639}{292.0}{ratebelow}
\DeliveryRow{1}{Kornia GPU}{9.44884112}{390.0}{ratebelow}
\DeliveryRow{2}{TorchVision CPU}{13.77624268}{330.0}{ratebelow}
\DeliveryRow{3}{Pillow}{14.59244950}{330.0}{ratebelow}
\DeliveryRow{4}{Pillow-AllSIMD (fast)}{15.36367449}{330.0}{ratebelow}
\DeliveryRow{5}{TorchVision GPU}{15.41628597}{544.0}{ratebelow}
\DeliveryRow{6}{AlbumentationsX}{17.12548000}{404.0}{ratereference}
\DeliveryRow{7}{DALI}{19.66780533}{1872.0}{rateabove}
}


==> generated/recipes.tex <==
% Generated by paper/generate_results.py. Do not edit by hand.
\hypertarget{R01}{\textbf{R01}} Resize & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic. \\
\hypertarget{R02}{\textbf{R02}} Random\allowbreak{}Crop224 & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image. \\
\hypertarget{R03}{\textbf{R03}} Random\allowbreak{}Resized\allowbreak{}Crop & \textbf{Random\allowbreak{}Resized\allowbreak{}Crop}: \texttt{size}=[224, 224]; \texttt{width}=224; \texttt{scale}=[0.08, 1.0]; \texttt{ratio}=[0.75, 1.3333333333333333]; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: per-image. \\
\hypertarget{R04}{\textbf{R04}} Random\allowbreak{}Crop224 $\to$ Horizontal\allowbreak{}Flip & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Horizontal\allowbreak{}Flip}: no parameters. Sampling: deterministic. \\
\hypertarget{R05}{\textbf{R05}} Random\allowbreak{}Crop224 $\to$ Vertical\allowbreak{}Flip & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Vertical\allowbreak{}Flip}: no parameters. Sampling: deterministic. \\
\hypertarget{R06}{\textbf{R06}} Pad $\to$ Random\allowbreak{}Crop224 & \textbf{Pad}: \texttt{padding}=10; \texttt{fill}=0; \texttt{border\_mode}="constant". Sampling: deterministic.\newline \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image. \\
\hypertarget{R07}{\textbf{R07}} Random\allowbreak{}Crop224 $\to$ Rotate & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Rotate}: \texttt{angle\_range}=[-45, 45]; \texttt{interpolation}="nearest"; \texttt{mode}="constant"; \texttt{fill}=0. Sampling: per-image. \\
\hypertarget{R08}{\textbf{R08}} Random\allowbreak{}Crop224 $\to$ Affine & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Affine}: \texttt{angle}=25.0; \texttt{shift}=[20, 20]; \texttt{scale}=2.0; \texttt{shear}=[10.0, 15.0]; \texttt{interpolation}="bilinear"; \texttt{mode}="constant"; \texttt{fill}=0; \texttt{reference\_size}=512. Sampling: per-image. \\
\hypertarget{R09}{\textbf{R09}} Random\allowbreak{}Crop224 $\to$ Perspective & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Perspective}: \texttt{scale}=[0.05, 0.1]; \texttt{interpolation}="bilinear"; \texttt{fill}=0. Sampling: per-image. \\
\hypertarget{R10}{\textbf{R10}} Random\allowbreak{}Crop224 $\to$ Elastic & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Elastic}: \texttt{sigma}=5.0; \texttt{torchvision\_alpha}=32.0; \texttt{kornia\_alpha}=0.14285714285714285; \texttt{displacement\_range}=[0.0097, 0.0097]; \texttt{control\_grid\_shape}=[29, 29]; \texttt{interpolation}="bilinear". Sampling: per-image. \\
\hypertarget{R11}{\textbf{R11}} Random\allowbreak{}Crop224 $\to$ Color\allowbreak{}Jitter & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Color\allowbreak{}Jitter}: \texttt{brightness}=0.5; \texttt{contrast}=1.5; \texttt{saturation}=1.5; \texttt{hue}=0.5. Sampling: per-image. \\
\hypertarget{R12}{\textbf{R12}} Random\allowbreak{}Crop224 $\to$ Channel\allowbreak{}Shuffle & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Channel\allowbreak{}Shuffle}: no parameters. Sampling: per-image. \\
\hypertarget{R13}{\textbf{R13}} Random\allowbreak{}Crop224 $\to$ Grayscale & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Grayscale}: \texttt{num\_output\_channels}=3. Sampling: deterministic. \\
\hypertarget{R14}{\textbf{R14}} Random\allowbreak{}Crop224 $\to$ RGBShift & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{RGBShift}: \texttt{pixel\_shift}=100. Sampling: per-image. \\
\hypertarget{R15}{\textbf{R15}} Random\allowbreak{}Crop224 $\to$ Gaussian\allowbreak{}Blur & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Gaussian\allowbreak{}Blur}: \texttt{sigma}=2.0; \texttt{kernel\_size}=[5, 5]. Sampling: per-image. \\
\hypertarget{R16}{\textbf{R16}} Random\allowbreak{}Crop224 $\to$ Gaussian\allowbreak{}Noise & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Gaussian\allowbreak{}Noise}: \texttt{mean}=0; \texttt{std}=0.44; \texttt{per\_channel}=true. Sampling: per-image. \\
\hypertarget{R17}{\textbf{R17}} Random\allowbreak{}Crop224 $\to$ Invert & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Invert}: no parameters. Sampling: deterministic. \\
\hypertarget{R18}{\textbf{R18}} Random\allowbreak{}Crop224 $\to$ Posterize & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Posterize}: \texttt{bits}=4. Sampling: deterministic. \\
\hypertarget{R19}{\textbf{R19}} Random\allowbreak{}Crop224 $\to$ Solarize & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Solarize}: \texttt{threshold}=0.5. Sampling: deterministic. \\
\hypertarget{R20}{\textbf{R20}} Random\allowbreak{}Crop224 $\to$ Sharpen & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Sharpen}: \texttt{alpha}=[0.2, 0.5]; \texttt{lightness}=[0.5, 1]. Sampling: per-image. \\
\hypertarget{R21}{\textbf{R21}} Random\allowbreak{}Crop224 $\to$ Auto\allowbreak{}Contrast & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Auto\allowbreak{}Contrast}: no parameters. Sampling: deterministic. \\
\hypertarget{R22}{\textbf{R22}} Random\allowbreak{}Crop224 $\to$ Equalize & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Equalize}: \texttt{mode}="pil". Sampling: deterministic. \\
\hypertarget{R23}{\textbf{R23}} Random\allowbreak{}Crop224 $\to$ Erasing & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Erasing}: \texttt{scale}=[0.02, 0.33]; \texttt{ratio}=[0.3, 3.3]; \texttt{fill}=0. Sampling: per-image. \\
\hypertarget{R24}{\textbf{R24}} Random\allowbreak{}Crop224 $\to$ Jpeg\allowbreak{}Compression & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Jpeg\allowbreak{}Compression}: \texttt{quality}=50. Sampling: per-image. \\
\hypertarget{R25}{\textbf{R25}} Random\allowbreak{}Crop224 $\to$ Random\allowbreak{}Gamma & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Random\allowbreak{}Gamma}: \texttt{gamma}=120. Sampling: per-image. \\
\hypertarget{R26}{\textbf{R26}} Random\allowbreak{}Crop224 $\to$ Plankian\allowbreak{}Jitter & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Plankian\allowbreak{}Jitter}: \texttt{mode}="blackbody". Sampling: per-image. \\
\hypertarget{R27}{\textbf{R27}} Random\allowbreak{}Crop224 $\to$ Median\allowbreak{}Blur & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Median\allowbreak{}Blur}: \texttt{blur\_limit}=5. Sampling: per-image. \\
\hypertarget{R28}{\textbf{R28}} Random\allowbreak{}Crop224 $\to$ Motion\allowbreak{}Blur & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Motion\allowbreak{}Blur}: \texttt{kernel\_size}=5; \texttt{angle\_range}=[0, 360]; \texttt{direction\_range}=[-1, 1]. Sampling: per-image. \\
\hypertarget{R29}{\textbf{R29}} Random\allowbreak{}Crop224 $\to$ CLAHE & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{CLAHE}: \texttt{clip\_limit}=[1, 4]; \texttt{tile\_grid\_size}=[8, 8]. Sampling: per-image. \\
\hypertarget{R30}{\textbf{R30}} Random\allowbreak{}Crop224 $\to$ Brightness & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Brightness}: \texttt{brightness\_limit}=[0.2, 0.2]. Sampling: per-image. \\
\hypertarget{R31}{\textbf{R31}} Random\allowbreak{}Crop224 $\to$ Contrast & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Contrast}: \texttt{contrast\_limit}=[0.2, 0.2]. Sampling: per-image. \\
\hypertarget{R32}{\textbf{R32}} Random\allowbreak{}Crop224 $\to$ Blur & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Blur}: \texttt{kernel\_size}=5; \texttt{border\_mode}="reflect". Sampling: per-image. \\
\hypertarget{R33}{\textbf{R33}} Random\allowbreak{}Crop224 $\to$ Channel\allowbreak{}Dropout & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Channel\allowbreak{}Dropout}: no parameters. Sampling: per-image. \\
\hypertarget{R34}{\textbf{R34}} Random\allowbreak{}Crop224 $\to$ Linear\allowbreak{}Illumination & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Linear\allowbreak{}Illumination}: \texttt{gain}=[0.01, 0.2]. Sampling: per-image. \\
\hypertarget{R35}{\textbf{R35}} Random\allowbreak{}Crop224 $\to$ Corner\allowbreak{}Illumination & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Corner\allowbreak{}Illumination}: \texttt{gain}=[0.01, 0.2]. Sampling: per-image. \\
\hypertarget{R36}{\textbf{R36}} Random\allowbreak{}Crop224 $\to$ Gaussian\allowbreak{}Illumination & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Gaussian\allowbreak{}Illumination}: \texttt{gain}=[0.01, 0.2]. Sampling: per-image. \\
\hypertarget{R37}{\textbf{R37}} Random\allowbreak{}Crop224 $\to$ Hue & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Hue}: \texttt{hue}=20. Sampling: per-image. \\
\hypertarget{R38}{\textbf{R38}} Random\allowbreak{}Crop224 $\to$ Plasma\allowbreak{}Brightness & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Plasma\allowbreak{}Brightness}: \texttt{roughness}=0.5. Sampling: per-image. \\
\hypertarget{R39}{\textbf{R39}} Random\allowbreak{}Crop224 $\to$ Plasma\allowbreak{}Contrast & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Plasma\allowbreak{}Contrast}: \texttt{roughness}=0.5. Sampling: per-image. \\
\hypertarget{R40}{\textbf{R40}} Random\allowbreak{}Crop224 $\to$ Plasma\allowbreak{}Shadow & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Plasma\allowbreak{}Shadow}: \texttt{roughness}=0.5. Sampling: per-image. \\
\hypertarget{R41}{\textbf{R41}} Random\allowbreak{}Crop224 $\to$ Rain & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Rain}: \texttt{drop\_width}=5; \texttt{drop\_height}=20; \texttt{brightness\_coefficient}=1.0. Sampling: per-image. \\
\hypertarget{R42}{\textbf{R42}} Random\allowbreak{}Crop224 $\to$ Salt\allowbreak{}And\allowbreak{}Pepper & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Salt\allowbreak{}And\allowbreak{}Pepper}: \texttt{amount}=[0.01, 0.06]; \texttt{salt\_vs\_pepper}=[0.4, 0.6]. Sampling: per-image. \\
\hypertarget{R43}{\textbf{R43}} Random\allowbreak{}Crop224 $\to$ Saturation & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Saturation}: \texttt{saturation\_factor}=0.5. Sampling: per-image. \\
\hypertarget{R44}{\textbf{R44}} Random\allowbreak{}Crop224 $\to$ Snow & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Snow}: \texttt{snow\_point\_range}=[0.5, 0.5]. Sampling: per-image. \\
\hypertarget{R45}{\textbf{R45}} Random\allowbreak{}Crop224 $\to$ Optical\allowbreak{}Distortion & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Optical\allowbreak{}Distortion}: \texttt{distort\_limit}=0.5; \texttt{mode}="fisheye". Sampling: per-image. \\
\hypertarget{R46}{\textbf{R46}} Random\allowbreak{}Crop224 $\to$ Shear & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Shear}: \texttt{shear}=10. Sampling: deterministic. \\
\hypertarget{R47}{\textbf{R47}} Random\allowbreak{}Crop224 $\to$ Thin\allowbreak{}Plate\allowbreak{}Spline & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Thin\allowbreak{}Plate\allowbreak{}Spline}: \texttt{num\_control\_points}=2; \texttt{distortion\_scale}=0.5. Sampling: per-image. \\
\hypertarget{R48}{\textbf{R48}} Random\allowbreak{}Crop224 $\to$ Photo\allowbreak{}Metric\allowbreak{}Distort & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Photo\allowbreak{}Metric\allowbreak{}Distort}: \texttt{brightness\_range}=[0.875, 1.125]; \texttt{contrast\_range}=[0.5, 1.5]; \texttt{saturation\_range}=[0.5, 1.5]; \texttt{hue\_range}=[-0.05, 0.05]. Sampling: per-image. \\
\hypertarget{R49}{\textbf{R49}} Random\allowbreak{}Crop224 $\to$ Color\allowbreak{}Jiggle & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Color\allowbreak{}Jiggle}: \texttt{brightness}=[0.875, 1.125]; \texttt{contrast}=[0.5, 1.5]; \texttt{saturation}=[0.5, 1.5]; \texttt{hue}=[-0.05, 0.05]. Sampling: per-image. \\
\hypertarget{R50}{\textbf{R50}} Longest\allowbreak{}Max\allowbreak{}Size $\to$ Random\allowbreak{}Crop224 & \textbf{Longest\allowbreak{}Max\allowbreak{}Size}: \texttt{max\_size}=512; \texttt{interpolation}="bilinear". Sampling: per-image.\newline \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image. \\
\hypertarget{R51}{\textbf{R51}} Smallest\allowbreak{}Max\allowbreak{}Size $\to$ Random\allowbreak{}Crop224 & \textbf{Smallest\allowbreak{}Max\allowbreak{}Size}: \texttt{max\_size}=512; \texttt{interpolation}="bilinear". Sampling: per-image.\newline \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image. \\
\hypertarget{R52}{\textbf{R52}} Random\allowbreak{}Crop224 $\to$ Transpose & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Transpose}: no parameters. Sampling: deterministic. \\
\hypertarget{R53}{\textbf{R53}} Random\allowbreak{}Crop224 $\to$ Random\allowbreak{}Rotate90 & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Random\allowbreak{}Rotate90}: \texttt{times}=[0, 3]. Sampling: per-image. \\
\hypertarget{R54}{\textbf{R54}} Random\allowbreak{}Crop224 $\to$ Random\allowbreak{}Jigsaw & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Random\allowbreak{}Jigsaw}: \texttt{grid}=[4, 4]. Sampling: per-image. \\
\hypertarget{R55}{\textbf{R55}} Random\allowbreak{}Crop224 $\to$ Enhance\allowbreak{}Edge & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Enhance\allowbreak{}Edge}: \texttt{mode}="edge"; \texttt{alpha\_range}=[0.5, 1.0]. Sampling: per-image. \\
\hypertarget{R56}{\textbf{R56}} Random\allowbreak{}Crop224 $\to$ Enhance\allowbreak{}Detail & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Enhance\allowbreak{}Detail}: \texttt{mode}="detail"; \texttt{alpha\_range}=[0.5, 1.0]. Sampling: per-image. \\
\hypertarget{R57}{\textbf{R57}} Random\allowbreak{}Crop224 $\to$ Unsharp\allowbreak{}Mask & \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image.\newline \textbf{Unsharp\allowbreak{}Mask}: \texttt{blur\_limit}=[3, 7]; \texttt{sigma\_limit}=0.0; \texttt{alpha}=[0.2, 0.5]; \texttt{threshold}=10. Sampling: per-image. \\
\hypertarget{R58}{\textbf{R58}} Center\allowbreak{}Crop & \textbf{Center\allowbreak{}Crop}: \texttt{height}=224; \texttt{width}=224. Sampling: deterministic. \\
\hypertarget{R59}{\textbf{R59}} Resize $\to$ Crop & \textbf{Resize}: \texttt{target\_size}=256; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Crop}: \texttt{top}=9; \texttt{left}=16; \texttt{height}=224; \texttt{width}=224. Sampling: deterministic. \\
\hypertarget{R60}{\textbf{R60}} Resize $\to$ Crop\allowbreak{}And\allowbreak{}Pad & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Crop\allowbreak{}And\allowbreak{}Pad}: \texttt{sides}=[-8, 12, 8, -12]. Sampling: deterministic. \\
\hypertarget{R61}{\textbf{R61}} Letter\allowbreak{}Box & \textbf{Letter\allowbreak{}Box}: \texttt{height}=224; \texttt{width}=224. Sampling: deterministic. \\
\hypertarget{R62}{\textbf{R62}} Pad\allowbreak{}If\allowbreak{}Needed $\to$ Random\allowbreak{}Crop224 & \textbf{Pad\allowbreak{}If\allowbreak{}Needed}: \texttt{min\_height}=256; \texttt{min\_width}=256. Sampling: deterministic.\newline \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image. \\
\hypertarget{R63}{\textbf{R63}} Resize $\to$ Channel\allowbreak{}Swap & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Channel\allowbreak{}Swap}: \texttt{channel\_order}=[2, 1, 0]. Sampling: deterministic. \\
\hypertarget{R64}{\textbf{R64}} Resize $\to$ Colorize & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Colorize}: \texttt{black}=[8, 24, 64]; \texttt{white}=[255, 238, 192]. Sampling: deterministic. \\
\hypertarget{R65}{\textbf{R65}} Resize $\to$ Dithering & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Dithering}: \texttt{method}="floyd\_steinberg"; \texttt{levels}=2. Sampling: deterministic. \\
\hypertarget{R66}{\textbf{R66}} Resize $\to$ Morphological & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Morphological}: \texttt{size}=3; \texttt{operation}="dilation". Sampling: deterministic. \\
\hypertarget{R67}{\textbf{R67}} Resize $\to$ Morphological & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Morphological}: \texttt{size}=3; \texttt{operation}="erosion". Sampling: deterministic. \\
\hypertarget{R68}{\textbf{R68}} Random\allowbreak{}Scale $\to$ Random\allowbreak{}Crop224 & \textbf{Random\allowbreak{}Scale}: \texttt{scale}=[0.75, 1.25]; \texttt{interpolation}="bilinear". Sampling: per-image.\newline \textbf{Random\allowbreak{}Crop224}: \texttt{height}=224; \texttt{width}=224. Sampling: per-image. \\
\hypertarget{R69}{\textbf{R69}} Resize $\to$ Random\allowbreak{}Sized\allowbreak{}Crop & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Random\allowbreak{}Sized\allowbreak{}Crop}: \texttt{crop\_size}=160; \texttt{input\_size}=224; \texttt{size}=[224, 224]. Sampling: per-image. \\
\hypertarget{R70}{\textbf{R70}} Resize $\to$ Coarse\allowbreak{}Dropout & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Coarse\allowbreak{}Dropout}: \texttt{hole\_size}=32; \texttt{input\_size}=224. Sampling: per-image. \\
\hypertarget{R71}{\textbf{R71}} Resize $\to$ Emboss & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Emboss}: \texttt{alpha}=0.5; \texttt{strength}=1.0. Sampling: deterministic. \\
\hypertarget{R72}{\textbf{R72}} Resize $\to$ Pixel\allowbreak{}Spread & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Pixel\allowbreak{}Spread}: \texttt{radius}=2. Sampling: per-image. \\
\hypertarget{R73}{\textbf{R73}} Resize $\to$ Shift\allowbreak{}Scale\allowbreak{}Rotate & \textbf{Resize}: \texttt{target\_size}=224; \texttt{interpolation}="bilinear"; \texttt{antialias}=false. Sampling: deterministic.\newline \textbf{Shift\allowbreak{}Scale\allowbreak{}Rotate}: \texttt{input\_size}=224; \texttt{angle}=12; \texttt{scale}=1.125; \texttt{shift}=[14, -7]. Sampling: deterministic. \\


==> generated/versions.tex <==
% Generated by paper/generate_results.py. Do not edit by hand.
AlbumentationsX & \texttt{2.6.3} \\
Pillow CPU & \texttt{13.0.0} \\
TorchVision CPU & \texttt{0.29.2} \\
TorchVision GPU & \texttt{0.29.2} \\
Kornia CPU & \texttt{0.9.1} \\
Kornia GPU & \texttt{0.9.1} \\
DALI GPU & \texttt{2.4.0} \\
Pillow-AllSIMD CPU (fast) & \texttt{13.0.0.post4} \\

